The Role of Conversation Context for Sarcasm Detection in Online Interactions

Computational models for sarcasm detection have often relied on the content of utterances in isolation. However, speaker's sarcastic intent is not always obvious without additional context. Focusing on social media discussions, we investigate two issues: (1) does modeling of conversation context help in sarcasm detection and (2) can we understand what part of conversation context triggered the sarcastic reply. To address the first issue, we investigate several types of Long Short-Term Memory (LSTM) networks that can model both the conversation context and the sarcastic response. We show that the conditional LSTM network (Rocktaschel et al., 2015) and LSTM networks with sentence level attention on context and response outperform the LSTM model that reads only the response. To address the second issue, we present a qualitative analysis of attention weights produced by the LSTM models with attention and discuss the results compared with human performance on the task.

==> qual_copy.tex <==
\subsection{Qualitative Analysis}

%One of the research goals in this work is to analyze whether it is possible to determine what part of the context (sentences for $IAC$; tweets for Twitter) triggers the sarcasm. In this section we visualize and discuss the attention patterns for the $IAC$ as well as for the tweets. 

Sarcasm is a complex phenomena in natural language and often humans too have low agreement on deciding if an utterance is sarcastic \cite{gonzalez,justo}. \newcite{wallace} showed that by providing  contextual information humans are able to identify sarcastic utterances which they were unable without the context. However, it is imperative to analyze what \textit{part of the context} triggers the sarcasm.    

We conducted a qualitative study by looking at the attention weights of the LSTM networks. We analyze which output representations the model is attending over when deciding the class of a sarcastic utterance. At the same time, we design a crowd-sourcing experiment to understand whether human annotators are also able to identify the contextual information that triggers a sarcasm. Below is a short description of the crowdsourcing experiment.

\paragraph{Crowdsourcing Experiment:}

We design an Amazon Mechanical Turk (for brevity, MTurk) task that given a pair of context $c$ and a sarcastic reply $r$ from the $IAC$, whether Turkers can identify part of the $c$ that may trigger the sarcasm in $r$. Our unit of analysis is sentences from the context. From the test data, we select examples with context length between three to seven sentences. For longer posts the MTurk task will be too complicated for the Turkers. We allowed the Turkers to chose one or multiple sentences that may trigger sarcasm in the reply post.

We provided definition of sarcasm and a couple of sarcastic examples of context-response pairs from $IAC$. Each HIT contains only one task and five Turkers were allowed to attempt each HIT. We selected Turkers with reasonable quality (i.e., more than 95\% of acceptance rate with experience of over 8,000 HITs) and paid seven cents per task. We visualize and discuss the attention patterns of the sentences in the context as well as Turkers' findings. Based on our observations of the attention weights as well as Turkers' choice we discuss some of the key findings in the following subsections. Figures \ref{figure:sentmap1} - \ref{figure:sentmap4}, represent the context-response pair in a table and the heat maps of the attention weights of sentences in the candidate context (LHS of the figure). The RHS represents the frequency of Turkers in choosing the particular sentence. Sentence numbers are in ``()''. Visualization of word-by-word attentions are depicted in Figures \ref{figure:wordmap1} - \ref{figure:wordmap4}. The top heatmap shows words from context $c$ whereas the bottom heatmap represents the response $r$. %all are correct %first sentence and then word


\begin{figure*}[t]
\centering
\begin{framed}
 \subfloat[\label{fig:hmap1}]
 {\includegraphics[width=1.7in]{heatmap_2_iac.png}}  \subfloat[ \label{fig:hmap2}]{\includegraphics[width=1.7in]{heatmap_1_iac.png}}
 \subfloat[ \label{fig:hmap3}]
 {\includegraphics[width=1.7in]{heatmap_3_iac.png}}
 \vskip 4ex
 \subfloat[\label{fig:hmap5}]
 {\includegraphics[width=1.7in]{heatmap_5_iac.png}}
 \subfloat[\label{fig:hmap4}]
 {\includegraphics[width=1.7in]{heatmap_4_iac.png}}
  \subfloat[\label{fig:hmap6}]
 {\includegraphics[width=1.7in]{heatmap_6_iac.png}}
 \end{framed}
 \centering
 \caption{Context sentences that trigger sarcasm in IAC corpus. LHS: \textit{attention weights}; RHS: \textit{Turkers' selections} (best in colors) }
 \label{figure:iachits}
\end{figure*}

\begin{figure*}[t]
\centering
\begin{framed}
 \subfloat[\label{fig:hmap21}]
 {\includegraphics[width=1.7in]{context_and_response1.png}} \hfil
 \subfloat[\label{fig:hmap23}]
 {\includegraphics[width=1.7in]{context_and_response2.png}}
 \end{framed}
 \centering
 \caption{Context sentences that trigger sarcasm in Tweets. (best in colors) }
 \label{figure:tweetshits}
\end{figure*}


% to show
% first - examples that match between turkers and weights
%example that do not match --
%tweet examples
%words, emoticons, etc. (indicator)
%factors?
\paragraph{Semantic coherence between context and response}
Figure \ref{figure:heatmap1} depicts a case where the context contains three sentences and the attention weights given to the sentences are similar to the Turkers' choice. Looking at this example, it seems the model pays attention to output vectors that are semantically coherent. Here, the sarcastic response (``\dots hold your tongue \dots in support of an anti-gay argument'') replies the action of the last sentence of the context (``\dots I've held my tongue on this \dots''). Our attention-based LSTM architecture is learning the attention weights simulteneously for the context $c$ and the response $r$. Thus the model is showing contextual understanding by setting high weights to semantically coherent parts of the $c$ and $r$. Similar to \cite{rocktaschel2015reasoning} we also observe that in many examples attention is capable of matching multi-word expressions, thus showing contextual understanding (example ``child'' and``three year old'' in Figure \ref{figure:wordmap2}).
%Sarcastic utterance remains sarcastic even with the removal of the marker. For example, capitalization of ``NEVER'' in ``A shooting in Oakland? That NEVER happens'', signals sarcasm, but removing the capitalization will not affect the presence of sarcasm (only its ease of recognition).
\paragraph{Role of sarcasm markers}
Sarcasm markers are explicit indicators of sarcasm that signal that an utterance is sarcastic. Such as the use of emoticons or uppercase spelling of words \cite{attardo2000irony,burgers2012verbal}.
 Use of such markers in social media (particularly in Twitter) is extensive. We observe in numerous examples attention weights prefer sentences containing sarcasm markers such as emoticons. For instance, in Figure \ref{figure:sentmap2}, highest weight is given to the sentence containing an emoticon for ``killing'' whereas from the response $r$, sentence with ``rolled eyes'' emoticon has received the highest attention. In other words, not only the model gives weights to the markers but also learn that such pair of opposite markers (i.e., killing face vs. rolled eyes) appear in context $c$ and its sarcastic response $r$.
 
\paragraph{Role of context incongruity}
A pre-condition for observing sarcasm is that the literal meaning of a sarcastic utterance is somehow incongruent with the context. This semantic incongruity is an inherent characteristic of irony and sarcasm and have been extensively studied in linguistics, philosophy, communication science \cite{attardo2000irony,camp2011,grice1975syntax,burgers2012verbal} as well as recently in NLP \cite{riloff,joshi2015}. For instance, \newcite{riloff} pointed out that identifying the incongruity between \textit{positive} sentiment expression and the \textit{negative} situation is a key characteristic of sarcasm detection in social media. We observe in $IAC$ and in Tweets, attention-based models have frequently identified sentences and words from $c$ and $r$ that are semantically incongruous (i.e., opposite sentiment words), thus helping in sarcasm detection. For instance in Figure \ref{figure:sentmap3} attention model has chosen S1 from context that contains strong negative sentiment word (``filthy disgusting \dots''). Interestingly, in contrast, attention model has given highest weight to opposite sentiment the response (``I love you'') with highest weight. Thus, the model seems to learn the context incongruity of opposite sentiment for sarcasm detection. From the perspective of the tweets, we observe often the sentence-based attention models have selected utterance(s) from the context which have opposite sentiment (``\dots not very christian of you'') to the respective sarcastic response (``\dots not very christian of you''). For the respective example, we observe ``christian'' and ``atheist'' received the highest weights (Figure \ref{figure:wordmap2}). The same behavior is also depicted in the case of Figure \ref{figure:wordmap3} and Figure \ref{figure:wordmap4}. Here, the word and sentence-level attention model have chosen the particular utterance from the context (i.e., the top heatmap for the context) and the words with high attention (``jew''; ``anti-semitic''), (``mediocre'',``gutsy''). These words again show examples of context incongruity which is useful for sarcasm detection. 

However, in complex scenarios, it is unclear whether identification of context incongruity guarantees understanding of sarcasm. For instance, in the Figure \ref{figure:sentmap3}, Turkers have chosen the S2 -- ``how can you tell a man that about his mum?'' -- as the most instructive sentence. \cite{rocktaschel2015reasoning} have argued that interpretations based on attentions weights have to be taken with care since the classification task is not forced to solely rely on only the attentions weights. Thus in future work, we plan to analyze utterances that are more subtle and do not consist of sarcasm indicators or explicit incongruence of opposite sentiment between context and response.


% Figure c), contains six sentences and we observe S2 is selected to have the highest attention as well as the most frequent choice from the Turkers. It is worthy to note, attention is able to identify the most informative sentence (i.e., ``\dots discussion on the national level would be a welcome change \dots bush administration wants to cut back on the prevention programs''). Besides, the last sentence in the context contains an URL and it has received the lowest attention value. In contrast, attention over the responses is more uniformly distributed. However, the penultimate sentence has got most attention and they are the sarcastic sentences in the response (i.e., ``\dots men are acting `recklessly' because they aren't treated as `normal'\dots'').    
%However, it is not always overlapping with Turker's choice. (deep mind note on judicial using of attention weights).



%Finally, in figure (f), attention weight preferred the last sentence that contains an emoticon for killing, where as the second choice (S1, the most informative sentence in the context post) is the preferred one from the Turkers. Similarly in the response post, the sentence with rolled eyes emoticon has received the highest attention. This example indicates that attention weight is given to sentences containing sarcasm markers \cite{burgers2012verbal} that assist in sarcasm classification. Whereas, Turkers have often chosen the sentence that is informative, with humor with subtle information.   
%understanding and detection is not the same thing!
%Moreover, attentions may be given to sarcasm indicators (i.e., features such as emoticons) that do not assist in \textit{understanding} the semantics of the dialogue. 
%Figure \ref{figure:tweethits} shows the heat map for the tweets. Recall, for tweets we treat each utterance separately. Also, $C_{i}$ are the context tweets where $C1$  
%is the original tweet that the sarcastic tweet replied. LHS shows how attention weight is distributed over the context utterances. 

%example of opposite sentiment (incongruence) 
%In this example, 

\begin{figure}[t]
\centering
 \subfloat[\label{fig:hmap21}]
 {\includegraphics[width=1.7in]{sent_context_disgust.png}} 
 \subfloat[\label{fig:hmap23}]
 {\includegraphics[width=1.7in]{heatmap_6_iac.png}}
 \centering
 \caption{Context sentences that trigger sarcasm in Tweets. (best in colors) }
 \label{figure:tweetshits}
\end{figure}



